Inferring the impact of feedback on the matter distribution using the Sunyaev Zel'dovich effect: Insights from CAMELS simulations and ACT+DES data

Feedback from active galactic nuclei and stellar processes changes the matter distribution on small scales, leading to significant systematic uncertainty in weak lensing constraints on cosmology. We investigate how the observable properties of group-scale halos can constrain feedback's impact on the matter distribution using Cosmology and Astrophysics with MachinE Learning Simulations (CAMELS). Extending the results of previous work to smaller halo masses and higher wavenumber, $k$, we find that the baryon fraction in halos contains significant information about the impact of feedback on the matter power spectrum. We explore how the thermal Sunyaev Zel'dovich (tSZ) signal from group-scale halos contains similar information. Using recent Dark Energy Survey (DES) weak lensing and Atacama Cosmology Telescope (ACT) tSZ cross-correlation measurements and models trained on CAMELS, we obtain $10\%$ constraints on feedback effects on the power spectrum at $k \sim 5\, h/{\rm Mpc}$. We show that with future surveys, it will be possible to constrain baryonic effects on the power spectrum to $\mathcal{O}(<1\%)$ at $k = 1\, h/{\rm Mpc}$ and $\mathcal{O}(3\%)$ at $k = 5\, h/{\rm Mpc}$ using the methods that we introduce here. Finally, we investigate the impact of feedback on the matter bispectrum, finding that tSZ observables are highly informative in this case.

==> backup.tex <==
\begin{comment}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h1_v4.pdf}
    \caption{Same as Fig.~\ref{fig:predict_v1}, but for showing information content of different parts of the pressure profile.  (a) suggests that knowing pressure at single point in profile contains lots of information about feedback, (b) previous results suggested that knowing integrating $Y$ doesn't help -- does this mean that feedback is not changing total thermal energy?}
    \label{fig:predict_v4}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h1_v5.pdf}
    \caption{Same as Fig.~\ref{fig:predict_v1}, but for showing information content of different parts of the number density profile.  }
    \label{fig:predict_v5}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h1_v6.pdf}
    \caption{Adding in cosmo info.  Reassuring that when we know all parameters, we do just about as well as we can.}
    \label{fig:predict_v6}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h1_vprof_vs_integrated.pdf}
    \caption{Profiles add more information than just integrated quantity.}
    \label{fig:predict_v7}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h1_vY500_cosmo.pdf}
    \caption{If you know $Y_{500}$ and cosmology, you can predict suppression pretty well.}
    \label{fig:predict_v8}
\end{figure*}


\clearpage

\section{High mass halos}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h2_v1.pdf}
    \caption{}
    \label{fig:predict_h2_v1}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h2_v2.pdf}
    \caption{}
    \label{fig:predict_h2_v2}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h2_v3.pdf}
    \caption{}
    \label{fig:predict_h2_v3}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h2_v4.pdf}
    \caption{}
    \label{fig:predict_h2_v4}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figs/predicting_pk_from_obs_h2_v5.pdf}
    \caption{}
    \label{fig:predict_h2_v5}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/Kai/Figure2.png}
    \caption{Prediction of the Astrophysical parameters of the simulation by a neural network using the Cosmological parameters and the pressure profiles of individual halos. The network seems to be able to predict the parameters of the simulation to some degree.}
    \label{fig:predict_astro}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/Kai/NeuronGradientAbs.png}
    \caption{Absolute neuron gradients for the neural network used for Figure \ref{fig:predict_astro} for each of the output neurons. The $11$ input parameters have been varied by some value and the resulting gradient was computed. The vertical red line separates the Cosmological information from the $9$ radial bins of the pressure profiles, where $1$ is the closest to the center of the halo. It seems that the network relies on the cosmological parameters for its predictions to a dominant degree. Out of the pressure profile information, only the innermost two seem to have a non-negligible contribution on the predicted values. This makes it likely that the network actually learns the Latin Hypercube configurations, instead of some underlying Physics.}
    \label{fig:predict_astro_gradient}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/Kai/nocosmo.png}
    \caption{Predictions of the same test set for an identical network architecture as used for \ref{fig:predict_astro}, but trained on the individual pressure profiles without the Cosmological information. The parameters can no longer be predicted to a reasonable degree. The feedback parameters could therefore not be learned from the individual halo pressure profiles.}
    \label{fig:predict_astro_no_cosmo}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/4layers_24_06_hist.png}
    \caption{Error of the predicted power spectrum residuals by the neural network using all input parameters and the Cosmological information. To avoid the learning of the Latin Hypercube as was the case in Figure \ref{fig:predict_astro}, all halos from randomly selected simulations were removed from the train set as opposed to just selecting random halos. This way the test set is solely comprised of LH configurations the network has not yet seen. It appears as if the network can predict the power spectrum for $k=.6,1.,10$ very well almost up to cosmic variance. The $k=.3$ predictions seems to be a little less accurate. (The mean absolute error for each k value is [0.0011822  0.00302704 0.00818195 0.02800818] (not weighted so it is expected that k=.3 is smaller even thought the plot looks worse)).}
    \label{fig:predict_res_nn}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/2_8_inputs_n_correct_legend.png}
    \caption{Error of the predicted power spectrum residuals using only the individual halo number density profiles (without Cosmological information).}
    \label{fig:predict_res_nn_n}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/2_8_inputs_p_correct_legend.png}
    \caption{Error of the predicted power spectrum residuals using only the individual halo pressure profiles (without Cosmological information). \eb{Is this actually individual halo pressure profiles, or mean across a mass bin?}}
    \label{fig:predict_res_nn_p}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/n+cosmo_astro.png}
    \caption{Prediction of Astrophysical parameters from mean number density profiles and Cosmological information. To prevent the learning of the LH configurations the test set was created using the same routine as in Figure \ref{fig:predict_res_nn}.}
    \label{fig:predict_astro_nn_n_mean+cosmo}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/p+cosmo_astro.png}
    \caption{Prediction of Astrophysical parameters from mean pressure profiles and Cosmological information. To prevent the learning of the LH configurations the test set was created using the same routine as in Figure \ref{fig:predict_res_nn}.}
    \label{fig:predict_astro_nn_p_mean+cosmo}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/n+cosmo_astro_individ.png}
    \caption{Prediction of Astrophysical parameters from individual number density profiles and Cosmological information. To prevent the learning of the LH configurations the test set was created using the same routine as in Figure \ref{fig:predict_res_nn}.}
    \label{fig:predict_astro_nn_n_individ+cosmo}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width =\textwidth]{figs/Kai/p+cosmo_astro_individ.png}
    \caption{Prediction of Astrophysical parameters from individual pressure profiles and Cosmological information. To prevent the learning of the LH configurations the test set was created using the same routine as in Figure \ref{fig:predict_res_nn}.}
    \label{fig:predict_astro_nn_p_individ+cosmo}
\end{figure*}

\end{comment}



\begin{comment}
\section{Main findings}

\begin{itemize}
    \item We confirm that baryon fraction contains lots of information about impact of feedback on matter power spectrum, even over wide range of feedback models relative to van Daalen, and for low mass halos, and for multiple cosmologies.  \eb{can we say something about the physical reason for this?}.  Seems that $f_b$ alone doesn't do very well -- need $f_b$ relative to cosmic.
    \item While we can use $f_b$ and profiles to predict impact of feedback, they don't constrain feedback parameters very well.  This implies that multiple combinations of feedback parameters can lead to same suppression.  \eb{is this true for all parameters?}. \eb{doesn't this contradict Moser et al. paper?}\todo{(1) try network using fewer layers/neurons, (2) Fisher matrix for feedback parameters with data being the mean pressure profile.}
    %\item Adding $Y_{500}$ and $n_{500}$ improves the constraints on power spectrum suppression a bit relative to knowing only $f_b$, particularly at high k.  This seems to be close to maximal information.  However, $f_b$ is difficult to measure.
    %\item $Y$ profile alone seems to do pretty well at predicting impact of feedback, adding $n$ profile helps a bit.  However with $Y$ profile alone, there seems to be a bit of a bias - can we understand this?  And $n$ profile seems to do better.  Maybe this comes from feedback injecting some thermal energy, decoupling $Y$ and changes to matter distribution?
    %\item Knowing the $Y$ profile does better than just knowing $Y_{500}$ (Fig. 7).  But this seems to only hold when cosmology is not known?    If cosmology is known, then knowing $Y_{500}$ alone does quite well.  Does this imply cosmology is degenerate with $Y_{500}$, but not with profile?  
    \item  Information content of Y profile \begin{itemize}
        \item  Y500 alone doesn't work very well, maybe because degenerate with cosmology
        \item Y500 + $\Omega_m$ does quite well, don't need sigma8, and don't need profile.  Is this weird?  Would be nice to not know cosmology. \todo{(1) Why does $\Omega_m$ impact $Y$? (2) re-plot $Y$-$M$ relation for different $\Omega_M$}
        \item combining Y500 with fb/cosmic improves performance at high k relative to fb/cosmic alone.  but there is no improvement in adding Y500 to fb+Om.
        \item y profile does better than Y500, and about as well as fb+Om
        \item y profile does about as well with cosmo as without
    \end{itemize}
    \item $f_b$ alone is not sufficient to predict impact of feedback because things also depend on cosmology.  We understand this dependnece is related to baryons split between multiple halos.   \eb{but why does changing $\Omega_m$ not significantly impact $f_b$ in some cases, even when number of halos is changing dramatically?}  Does this explanation actually work?  seems to be sensitivte to halo mass.  Does van daalen explain
        \begin{itemize}
            \item Impact of cosmology on $f_b$ seems to be very sensitive to halo mass range
        \end{itemize}
    \item Model from Simba does not work for illustris, and vice versa.  However, it is possible to train a model that works for both.  \eb{what is difference between these models?}
\end{itemize}



\section{Remaining questions}

\begin{itemize}
    \item Is measurement of $\Delta P$ robust if we're missing high-mass halos?  \todo{Understand the $dP/dM$ plot better  - is there a better plot?}
    \item figure out plots
    \item Try RF with individual profiles? Instead: train on mean profile, and variance profile
    \item Try neural network with mean profile? Done - doesn't work so well
    %\item do RF predictions on 1P
    %\item Why does knowing cosmology and $Y_{500}$ seem to do so well at predicting feedback suppression?  Why does knowing cosmology improve constraints from $Y_{500}$ alone?  \eb{Seems to imply that changing cosmology preserves $Y_{500}$, but changes profile.  So knowing profile breaks degeneracy between cosmology and $Y_{500}$, and knowing cosmology also breaks this degeneracy}
    %\item understand weird population of halos at high $\Omega_m$
    %\item how does $f_b$ alone vs. $f_b$+cosmology do?  cosmology is somewhat degenerate with $f_b$
    %\item try RF predicting $\Delta P/P$ given just sigma8 - this should be shit says Shivam \eb{This doesn't really seem to be the case - $\Omega_m$ and $\sigma_8$ both lead to roughly the same constraint}
    %\item Random forest on mean profiles to predict feedback parameters.  Has this been done? \eb{Did this, and RF cannot predict feedback parameters}
    %\item $\Delta P/P$ to feedback parameters.  \eb{works pretty shit}
    %\item plot $\Delta P /P$ as function of $k$ for multiple cosmologies and feedback sets: does this actually depend on cosmology?  is there some k for which the sensitivity to feedback is higher than to cosmology
    %\item Plot $\Delta P /P$ using Mead model as a function of $\sigma_8$.
    %\item Plot $\Delta P$ vs. $\Omega_m$ and $\sigma_8$
    %\item redo with SIMBA  \todo{redo RF stuff with this}
    %\item redo RF and neural network stuff using lower mass halos  \eb{present two different bins?}
    %\item Train network on mean profiles to predict $\Delta P$.  Done.
    %\item train on individual profiles to predict $\Delta P$.  Done.
    %\item Train on mean profiles to predict feedback parameters.  Has this been done?
    %\item Repeat all this with SIMBA?
    %\item there seems to be a bias for lowest $k$ bin
    %\item Are these tests with random forest regression sufficient, or should we do some neural network approach?
    \item Where is information in profile coming from?
    %\item Some way to include information from multiple individual halos?
    \item is knowing impact on $P(k)$ to 25\% sufficient for future surveys?
    \item compare to DES constraints - we have measurement of $Y_{500}$, can we turn this into constraint on feedback?
    \item How difficult is it to measure $f_b$?  Combine ksz with lensing?
    \item how do measurement errors impact findings?
    %\item Try 2D map instead of 1d profile?
    %\item \eb{Try Y500 in two different mass bins?}
    %\item Why does $Y_{500}$ + $\Omega_m$ work so well?  Slightly scary, since we don't really want to be learning about power spectrum
    %\item Do we want to predict full $\Delta P(k)$ rather than just at a single $k$ value?  Could PCA $\Delta P$ and predict amplitude of coefficient
    %\item understand changes to profiles from changing cosmological parameters.  The most massive halos have $f_b = \Omega_b/Omega_m$, since they form from representative parts of the Universe.  By increasing $\sigma_8$, we form more massive halos, meaning that there's fewer baryons to be in the small halos, leading to decrease in pressure?
    %\item use RF to get feedback parameters from profiles
\end{itemize}


\end{comment}


\section{Fisher matrix}


\begin{equation}
    F_{ij} = \frac{d P}{d \Delta_{p,i}} C^{-1}\frac{d P}{d \Delta_{p,j}} 
\end{equation}

\begin{equation}
    \frac{dP}{d \Delta_p} = \sum_i \frac{\partial P}{\partial \theta_i} \frac{\partial \theta_i}{\partial \Delta_p}
\end{equation}


\begin{eqnarray}
    \frac{\Delta P}{P_{\rm DMO}} &=& %-2\frac{M_{\rm ej}}{M} \\
    -2 \frac{f_c (\Omega_b/\Omega_m) M - cY/T -M_0}{M} \\
    &=& -2\frac{f_c\Omega_b}{\Omega_m} \left(1 - \frac{cY \Omega_m}{f_c TM \Omega_b} - \frac{M_0 \Omega_m}{f_c M\Omega_b} \right) .
%    &=& -2\frac{f_c\Omega_b}{\Omega_m} \left(1 - \frac{dY \Omega_m}{f_c M^{5/3} \Omega_b} - \frac{M_* \Omega_m}{f_c M\Omega_b} \right) 
\end{eqnarray}

when $Y$ is very small, we should have $\Delta P/ P \sim -2 f_c \Omega_b/\Omega_m - M_0/M$.  We should also have $Y/Y^{\rm SS} = f_c - M_0\Omega_m/(M \Omega_b)$ when $\Delta P/P = 0$.  In this simple model, the connection between these points will be a linear function of $Y/Y^{\rm SS}$.  When the halo mass is very large, we expect $f_c = 1$ and $M_0/M_{\rm gas} = 0$, so the model will linearly interpolate between $(\Delta P/P,Y/Y^{\rm SS}) = (-2\Omega_b/\Omega_m,0)$ and $(\Delta P/P,Y/Y^{\rm SS}) = (0,1)$.  This linear relation is shown with the dashed line in the $Y$ columns of Figs.~\ref{fig:Y_fb_DeltaP} and in \ref{fig:scatter_plot_all_ks}.  At smaller halo mass, $f_c < 1$ and $M_0/M$ will become significant.

We can also write 
\begin{eqnarray}
    M_{\rm ej} &=& f_c(\Omega_b/\Omega_m)M  - f_{b} M - M_0,
\end{eqnarray}
(where $f_b$ includes stellar mass following van Daalen) which leads to
\begin{eqnarray}\label{eq:DelP_P_fb}
    \frac{\Delta P}{P_{\rm DMO}} = -2 \frac{f_c\Omega_b}{\Omega_m} \left( 1 -\frac{f_{b}\Omega_m}{f_c \Omega_b}  - \frac{\Omega_m M_0}{f_c \Omega_b M} \right).
\end{eqnarray}
In other words, we find a linear relation between $\Delta P/P_{\rm DMO}$ and $f_b \Omega_m/\Omega_b$ with endpoints at $(\Delta P/P_{\rm DMO},f_b \Omega_m/\Omega_b) = (-2\Omega_b/\Omega_m,0)$ and $(\Delta P/P_{\rm DMO},f_b \Omega_m/\Omega_b) = (0,1)$ for high-mass halos.  This relation is shown as the dashed line in the $f_b$ columns of Figs.~\ref{fig:Y_fb_DeltaP}.

==> notes <==
\begin{itemize}
    \item ``We note here that the power spectrum is changed by
feedback rearranging matter – primarily gas –around galaxies, in some cases out to beyond the virial radius. While the
positions of galaxies and haloes may change as well when
baryons are added or feedback is varied, van Daalen et al.
(2014) have shown that this does not drive the shifts in the
power spectrum. Furthermore, note that the power spectrum changes on scales larger than the maximum scale over
which matter is displaced in real space. In the language of
the halo model, feedback changes the large-scale power by
decreasing the 2-halo term in a mass-dependent way''
    \item backreaction on cdm
    \item Without winds driven by
stellar feedback, the (self-regulated) AGN has a larger reservoir of cold gas at its disposal, and both accretes and heats
far more gas (leading to much more massive supermassive
black holes as well). Consequently, it is able to suppress the
matter clustering to a much larger degree, largely compensating for the strong increase in star formation in low-mass
galaxies. This agrees with Booth Schaye (2013), who used
OWLS to demonstrate that stellar feedback diminishes the
effectiveness of AGN feedback. This result also shows why
the bahamas heating temperature needed to go down to
match observations after reducing the stellar feedback: less
gas ejected by stars means more gas is available to the AGN,
making it more effective at a fixed heating temperature.
\item stellar
feedback determines what gas remains in a galaxy, to be
heated by an AGN once the galaxy is sufficiently massive to
host it (e.g. Bower et al. 2017). It is important, in order to
predict the right amount of power suppression due to AGN,
that the strength of stellar feedback is correctly calibrated to
observations as well. Calibrating only AGN feedback using
hot gas fractions in addition to the high-mass SMF may or
may not be enough; further research is needed for this.
\item We note
that this does not apply to the power spectra themselves:
while not shown here, the matter power spectra of each resimulated volume show random variations which can reach 10\% even on large scales – however, the ratio of power
spectra with and without baryons in the same volume is
converged to high precision
\item baryon fraction vs. gas fraction - baryon fraction very difficult to measure
\item  the problem with this is that in the absence of
strong feedback, the galaxies overcool and convert the gas
into stars instead, leading to a low gas fraction but no
suppression of power on large scales \eb{this doesn't seem to be happening in our stuff?}
\item Where this gas is distributed to should
not be relevant at the 1\% level on large scales, just that it
is removed from clustered regions – after all, unless feedback moves matter over distances 10 Mpc, changing
the mass of clustered regions is the only way to significantly
change the power for k 1 h . Because of this, we
might expect to be able to model the power suppression
on large scales as a function of only the baryon fraction in
group-sized haloes, which dominate the change in clustering.
\item check van Daalen fitting function against our results?
\item Beyond k 1 h Mpc1,however, this approximation fails. This is because on these
scales the power spectrum is sensitive to the changes in the
internal structure of group-sized haloes, which requires additional modelling. In halo model terms, for k 1 the power spectrum is sensitive to the 1halo term of 1014
haloes, while its contribution is constant for k1
(e.g. Debackere, Schaye Hoekstra 2019)
\item We find that
the mean baryon fraction of these haloes is more strongly
correlated with the suppression of power than that of haloes with masses around 1013 M or 1015
\end{itemize}



\begin{comment}


Since we assume that the ejected gas mass doesn't cluster, we can write the overdensity in the baryons as
\begin{equation}
    \delta_b' = \delta_b(1- M_{\rm ej}/M_{b}),
\end{equation}
where the unprimed $\delta_b$ indicates the overdensity without feedback, $M_{\rm ej}$ is the mass of gas that gets ejected from the halos, and $M_{\rm b}$ is the mass in baryons in the halos in the absence of feedback.

We then have
\begin{eqnarray}
    \frac{\delta_m'}{\delta_m} &=& \frac{\delta_c + \delta_b'}{\delta_c + \delta_b} = 1 - \frac{\delta_b M_{\rm ej}/M_{b}}{\delta_m} \\
    &=& 1 - \frac{\Omega_b M_{\rm ej}}{\Omega_m M_{b}}
\end{eqnarray}
and the power spectrum becomes
\begin{eqnarray}
    P' &=& P\left(1-\frac{ \Omega_b M_{\rm ej}}{\Omega_m M_{b}} \right)^2 \\
    &\approx& P\left(1-2\frac{ \Omega_b M_{\rm ej}}{\Omega_m M_{b}} \right).
\end{eqnarray}
So 
\begin{eqnarray}
    \frac{\Delta P}{P} = -2\frac{\Omega_b M_{\rm ej}}{\Omega_m M_{b}} .
\end{eqnarray}

Now, we can re-write this in terms of $Y$ and in terms of $f_b$.  We have
\begin{eqnarray}
    \frac{cY}{T} = M_{b} - M_{\rm ej} - M_*,
\end{eqnarray}
where $T$ is the gas temperature and $c$ is some constant (that depends on volume of the halo).  Substituting into the above we have
\begin{eqnarray}
    \frac{\Delta P}{P} &=& -2\frac{f_c \Omega_b}{\Omega_m} \left( 1- \frac{Yc}{T M_{b}} - \frac{M_*}{M_{b}} \right)  \\
\end{eqnarray}
Using $M_{b} \propto f_c \Omega_b M / \Omega_m$ and $T\propto M^{2/3}$, we have
\begin{eqnarray}
    \frac{\Delta P}{P} &=& -2\frac{f_c \Omega_b}{\Omega_m} \left( 1- \frac{dY\Omega_m}{f_c \Omega_b M^{5/3} } - \frac{M_* \Omega_m}{M f_c \Omega_b} \right),
\end{eqnarray}
where $d$ is some constant.  This seems reasonable compared to the plots.

Alternatively, we can define the self-similar $Y$ as $Y^{SS}c/T = M_{\rm gas} = M_b - M_*$ (i.e. it's what we expect without feedback).  Then we have $M_b = Y^{SS} c/T + M_*$, and 
\begin{eqnarray}
        \frac{\Delta P}{P} &=& -\frac{2f_c \Omega_b}{\Omega_m} \left( 1-\frac{Y}{Y^{SS} + M_*T/c} - \frac{M_* \Omega_m}{M f_c \Omega_b} \right) \\
        &=& -\frac{2f_c \Omega_b}{\Omega_m} \left( 1-\frac{Y}{Y^{SS} (1 + M_*/M_{\rm gas})} - \frac{M_* \Omega_m}{M f_c \Omega_b} \right) \nonumber \\
\end{eqnarray}
This has the expected behavior that when $Y$ is equal to its self-similar value, $\Delta P/P = 0$.

We can also write 
\begin{eqnarray}
    M_{\rm ej} &=& M_{b} - M_{\rm gas} - M_* = M_b - f_{b} M   \\
    &=&  M_{b} - f_{b} M_{b} (\Omega_m/f_c\Omega_b),
\end{eqnarray}
(where $f_b$ includes stellar mass following van Daalen) which leads to
\begin{eqnarray}
    \frac{\Delta P}{P} = -2 \frac{f_c \Omega_b}{\Omega_m} \left( 1-\frac{f_{b}\Omega_m}{f_c \Omega_b}  \right).
\end{eqnarray}
\end{comment}
